Understanding Visual Concepts with Continuation Learning

We introduce a neural network architecture and a learning algorithm to produce factorized symbolic representations. We propose to learn these concepts by observing consecutive frames, letting all the components of the hidden representation except a small discrete set (gating units) be predicted from the previous frame, and let the factors of variation in the next frame be represented entirely by these discrete gated units (corresponding to symbolic representations). We demonstrate the efficacy of our approach on datasets of faces undergoing 3D transformations and Atari 2600 games.

==> makefile <==
all: html pdf

pdf:
	pandoc main.md \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		--template pandoc_template.tex \
		-o output/rendered.pdf

tex:
	pandoc main.md \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		--template pandoc_template.tex \
		-o rendered.tex
html:
	pandoc main.md \
		--filter pandoc-crossref \
		--filter pandoc-citeproc \
		-s \
		--to html5 \
		-o output/rendered.html --mathjax

watch:
	reload -b -s output/rendered.html & make html & fswatch -o *.md */*.md | xargs -n1 make html

